MAPLE: Multilingual Evaluation of Parameter Efficient Finetuning of Large Language Models

Parameter Efficient Finetuning (PEFT) has emerged as a viable solution for improving the performance of Large Language Models (LLMs) without requiring massive resources and compute. Prior work on multilingual evaluation has shown that there is a large gap between the performance of LLMs on English and other languages. Further, there is also a large gap between the performance of smaller open-source models and larger LLMs. Finetuning can be an effective way to bridge this gap and make language models more equitable. In this work, we finetune the LLama-2-7B and Mistral-7B models on two synthetic multilingual instruction tuning datasets to determine its effect on model performance on six downstream tasks covering forty languages in all. Additionally, we experiment with various parameters, such as rank for low-rank adaptation and values of quantisation to determine their effects on downstream performance and find that higher rank and higher quantisation values benefit low-resource languages. We find that PEFT of smaller open-source models sometimes bridges the gap between the performance of these models and the larger ones, however, English performance can take a hit. We also find that finetuning sometimes improves performance on low-resource languages, while degrading performance on high-resource languages.

==> discussions.tex <==
\section{Analysis of Results}

\paragraph{RQ1: How does LoRA Rank and Quantisation Affect Model Performance?}

We observe that on an average, there is no particular trend of model performance on our tasks when it comes to increase in rank or quantisation. However, we can observe a consistently good score on an average when the models are finetuned on rank between 32 and 64 with 8 bit quantisation. 4 bit quantisation works well with lower ranks and 16 bit works well with higher ranks. We plot these findings in Figures \ref{fig: xnli model average},  \ref{fig: xquad model average}, \ref{fig: xcopa model average}, \ref{fig: belebele model average} and \ref{fig: mlqa model average}. 

For XNLI, we observe there is no particular trend with increasing quantisation and rank. For XCOPA, we observe that 4bit quantisation does well with lower rank and 16bit quantisation works well with higher ranks. For Belebele, we observe that higher quantisation yields better results. For MLQA, we observe that higher rank and higher quantisation leads to best performance. In XQUAD, 8 bit quantization does well with rank 64 and 16 bit outperforms every other setting with rank 128. \textbf{Overall, it is always the best to finetune models with highest rank and quantisation if possible, however, lower ranks and quantisation can turn out to be promising in some scenarios}. 

\paragraph{RQ2: How does quantisation affect the Performance of multilingual finetuned models across ranks?}

We observe that performance does not get affected by change in quantisation in \llm\ while in \mis\ we observe large fluctuations in performance as the quantisation changes for each rank. We also observe that \textbf{lower resource languages perform poorly in the lower quantisation settings}. We illustrate this in Figures \ref{fig: xnli quant vs rank fig}, \ref{fig: xcopa quant vs rank fig}, \ref{fig: belebele quant vs rank fig}, \ref{fig: mlqa quant vs rank fig} and \ref{fig: xquad quant vs rank fig}.

We observe that XNLI does not have an obvious trend, while the other datasets show no effect of quantisation on languages. \textbf{We also observe that \llm\ is more immune to change in fluctuation on quantisation across languages while \mis\ is more sensitive to quantisation across languages.}

\paragraph{RQ3: How does rank affect the performance of multilingual finetuned models across different values of quantisation?}


There is a direct correlation of performance with rank in most cases. We also observe that \textbf{lower resource languages are benefited the most by finetuning using higher ranks}. We illustrate these trends in detail in Figures \ref{fig: xnli model average per rank}, \ref{fig: xcopa model average per rank}, \ref{fig: belebele model average per rank}, \ref{fig: mlqa model average per rank} and \ref{fig: xquad model average per rank}.

We see that variation of rank across quantisations does not lead to any change in a particular language's performance in \llm\ i.e. varying rank across on any quantisation leads to same trends for all datasets. However in \mis\ there is no apparent trend in rank variation across quantisations unlike \llm\ . 



\paragraph{RQ4: Does Multilingual PEFT result in better downstream task performance compared to models that are not finetuned?}

In Figure \ref{fig: comparitive model average} we can see that finetuning is usually better or at par with LlaMA-70B-Chat and and Mistral-7B-Instruct which are not finetuned on multilingual data. We also compare the performance of finetuned models with LLMs like GPT-4 and PaLM2 and English instruction tuned versions of these models provided in \cite{ahuja2023megaverse} in Table \ref{tab:taskwise_average_results}, which shows averages across languages per tasks. We find that for tasks such as XCOPA and XQUAD, PEFT is able to bridge the gap to a large extent between open source and closed models, with PEFT Mistral's performance on XQuaD exceeding that of GPT-4 and PaLM2. However, for other datasets, we observe a degradation or no change, which could be attributed to test data contamination, or a regression on languages of the datasets. Datasets such as XNLI contain a large number of languages (Bulgarian, Greek, English, Hindi, Swahili, Turkish, Urdu, Chinese) that are not present in the MultiAlpaca dataset, which could explain the poor performance on the PEFT models on this downstream task.


We illustrate language wise analysis in Figures \ref{fig: xnli langwise model average}, \ref{fig: xcopa langwise model average}, \ref{fig: belebele langwise model average}, \ref{fig: mlqa langwise model average} and \ref{fig: xquad langwise model average}. 

For XNLI and MLQA, we observe that finetuning improves performance on low resource languages but worsens performance on high resource languages. In Belebele, we find that finetuning worsens the performance for all languages for both models. For XCOPA, we get the same or better results for all languages with finetuning. For XQUAD, multilingual finetuning boosts performance for all languages for both \llm\ and \mis\ . \textbf{This shows that PEFT on smaller LLMs on multilingual instruction data can prove to be beneficial and can bridge the gap between smaller open source models and large proprietary models for multilingual applications for some downstream applications}. 

While we compare our multilingual finetuned models with models finetuned on English, we should note that we do not have complete information about instruction datasets used for Llama-70B-chat and Mistral-7B-Instruct. Hence, there may be chances of data contamination for some datasets in these models \cite{ahuja-etal-2023-mega} or the presence of multilingual instruction data in them.

\paragraph{RQ5: How much loss is observed in performance on English due to multilingual finetuning?}


Finetuning LLMs on multilingual data leads to significant loss in performance on English where the score reduces by 90\% of base \llm\ and 50\% of \mis\ . On evaluating with the Alpaca Eval benchmark, all finetuned models significantly worse than the base models. However, we  observe that higher quantisation and higher rank on an average helps preserve the English performance to some extent. We illustrate trends with rank and quantisation of our finetuned model in Figures \ref{fig: alpaca eval rank analysis} and \ref{fig: alpaca eval quant analysis}.


